Optimal Energy Management in Autonomous Power Systems with Probabilistic Security Constraints and Adaptive Frequency Control

The decarbonization of many heavy power-consuming industries is dependent on the integration of renewable energy sources and energy storage systems in isolated autonomous power systems. The optimal energy management in such schemes becomes harder due to the increased complexity and stability requirements, the rapidly varying operating conditions and uncertainty of renewable sources, the conflicting objectives across different timescales, the limited amount of reliable power sources and energy storage. The state of charge management when energy storage is used for multiple services, such as optimal scheduling and frequency support, is one of the most notorious problems in this context. To address this issue, an optimal energy management system is proposed in this paper. It co-optimizes the primary frequency control layer and the dispatch schedule of conventional generators and energy storage by taking advantage of an algorithm that provides adaptive active power demand uncertainty quantification, theoretical guarantees for frequency stability, and bounds for the reserves for frequency support assigned to the energy storage system. A convex reformulation is derived enabling the efficient solution of the involved optimization problem, being a test case of an isolated offshore oil and gas platform presented for validation.

==> Manuscript/Acknowledgement.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}

Project / research funded by VISTA - a basic research program in collaboration between The Norwegian Academy of Science and Letters, and Equinor.

This scientific paper was supported by the Onassis Foundation - Scholarship ID: F ZP 056-1/2019-2020 and by the Research Council of Norway under the program PETROMAKS2, grant number 281986, project ``Innovative Hybrid Energy System for Stable Power and Heat Supply in Offshore Oil and Gas Installation (HESOFF)”.

==> Manuscript/Nomenclature.tex <==
% ----------------------THIS IS FROM J1. NEED TO CHANGE----------------------------------
%----------------------------------------------------------------------------------------
%% This code creates the groups
% -----------------------------------------
\renewcommand\nomgroup[1]{%
  \item[\bfseries
  \ifstrequal{#1}{A}{Sets}{%
  \ifstrequal{#1}{B}{Datasets}{%
  \ifstrequal{#1}{C}{Optimization variables and parameters}{%
  \ifstrequal{#1}{D}{Uncertainty modelling}{%
  \ifstrequal{#1}{E}{Power system variables}{}}}}}%
]}
% -----------------------------------------

% \mbox{}

\hl{
\nomenclature[A,02]{$g \in N_G$}{Generator units}
\nomenclature[A,01]{$t \in T$}{Time periods}
\nomenclature[A,03]{$\bm{\widetilde{\xi}}(\omega) \in \Omega$}{Uncertainty space}
\nomenclature[A,04]{$\bm{\widehat{\xi}}(\omega) \in \Omega_s$}{Reduced scenarios subsets}
\nomenclature[A,05]{$\bm{\widehat{\xi}}(\omega) \in \Omega_s^*$}{Optimally reduced scenarios subset}

\nomenclature[B,01]{$\left \{ \xi^{\ell} \right \}_{i=1:N}$}{system aggregated load}
\nomenclature[B,02]{$\left \{ \xi^{\textit{w}} \right \}_{i=1:N}$}{wind speed}

\nomenclature[C,01]{$\bm{x}$}{first stage decision variables}
\nomenclature[C,02]{$\bm{y}$}{second stage decision variables}
\nomenclature[C,03]{$\bm{c}$}{first stage cost}
\nomenclature[C,04]{$\bm{q}$}{second stage cost}
\nomenclature[C,06]{$\pi_\omega$}{scenario probability}

\nomenclature[D,01]{$\bm{\widetilde{\xi}}$}{sampled stochastic process}
\nomenclature[D,02]{$\bm{\widehat{\xi}}$}{scenarios (reduced uncertainty space)}
\nomenclature[D,03]{$\widehat{\xi}_t^{\ell}$}{load scenario at time $t$}
\nomenclature[D,04]{$W \left( \widehat{\xi}_t^w\right)$}{wind power scenario at time $t$}
\nomenclature[D,05]{$\widehat{F}^{\ell}_{h,t}(\tilde{\xi}_t^\ell)$}{marginal empirical cdf for load at time $t$}
\nomenclature[D,06]{$\widehat{F}^{\textit{w}}_{h,t}(\tilde{\xi}_t^\textit{w})$}{marginal empirical cdf for wind speed at time $t$}
\nomenclature[D,07]{$F^{\ell}\left(\widetilde{\bm{\xi}}^{\ell}\right)$}{multivariate joint distribution for load}
\nomenclature[D,08]{$F^{\textit{w}}\left(\widetilde{\bm{\xi}}^{\textit{w}}\right)$}{multivariate joint distribution for wind speed}

\nomenclature[E,01]{$P_{GT,t,\omega}^g$}{gas turbine power at time $t$}
\nomenclature[E,02]{$u_{t,\omega}^g $}{gas turbine ON/OFF status at time $t$}
\nomenclature[E,03]{$z_{t,\omega}^g$}{gas turbine startup command at time $t$}
\nomenclature[E,04]{$R$}{gas turbine ramping rate}
\nomenclature[E,05]{$P_{D,t,\omega}$}{controllable dumping power at time $t$}
\nomenclature[E,06]{$P_B$}{energy storage power rating}
\nomenclature[E,07]{$E_B$}{energy storage capacity rating}
\nomenclature[E,08]{$P_{B,t,\omega}$}{energy storage power at time $t$}
\nomenclature[E,09]{$E_{B,t,\omega}$}{energy storage charge level at time $t$}
}

\printnomenclature
